Mitigating Temporal-Drift: A Simple Approach to Keep NER Models Crisp

Performance of neural models for named entity recognition degrades over time, becoming stale. This degradation is due to temporal drift, the change in our target variables' statistical properties over time. This issue is especially problematic for social media data, where topics change rapidly. In order to mitigate the problem, data annotation and retraining of models is common. Despite its usefulness, this process is expensive and time-consuming, which motivates new research on efficient model updating. In this paper, we propose an intuitive approach to measure the potential trendiness of tweets and use this metric to select the most informative instances to use for training. We conduct experiments on three state-of-the-art models on the Temporal Twitter Dataset. Our approach shows larger increases in prediction accuracy with less training data than the alternatives, making it an attractive, practical solution.

==> figures/case_study.tex <==
\begin{table*}[t!]
% \small
\resizebox{\linewidth}{!}{
\begin{tabular}[t]{@{}llll@{}}
\toprule
\textbf{\#} 
    & \textbf{Sentence} 
    & \textbf{Entities} 
    & \textbf{Trending N-grams} 
\\\midrule
1 & 
\begin{tabular}[t]{@{}p{0.7\linewidth}@{}}
    Graduation has been set!! The \textbf{{[}SHS{]}\sub{facility}} CLASS OF 2015 will graduate on June 18th, 6:00 p.m. at \textbf{{[}Penders Field{]}\sub{facility}}! 
\end{tabular} & 
\begin{tabular}[t]{@{}l@{}}
    {[}SHS CLASS{]}\sub{other}\\
    {[}Penders Field{]}\sub{facility}
\end{tabular} & 
{[}Penders Field{]}\sub{facility} 
\\\midrule
2 & 
\begin{tabular}[t]{@{}p{0.7\linewidth}@{}}
    On another hand, \textbf{{[}Mayim{]}\sub{person}} will be guesting on \textbf{{[}Access Hollywood Live{]}\sub{tvshow}} tomorrow ! 
\end{tabular} & 
\begin{tabular}[t]{@{}l@{}}
    {[}Mayim{]}\sub{person} \\
    {[}Access Hollywood Live{]}\sub{tvshow}
\end{tabular} & 
\begin{tabular}[t]{@{}l@{}}
    {[}Mayim{]}\sub{person} \\ 
    {[}Access Hollywood{]}\sub{other}
\end{tabular} 
\\\bottomrule
\end{tabular}
}
\caption{The case studies of n-grams that identified as trending topics. }
\label{tab:case_study}
\end{table*}

